Syn3DTxt: Embedding 3D Cues for Scene Text Generation

This study aims to investigate the challenge of insufficient three-dimensional context in synthetic datasets for scene text rendering. Although recent advances in diffusion models and related techniques have improved certain aspects of scene text generation, most existing approaches continue to rely on 2D data, sourcing authentic training examples from movie posters and book covers, which limits their ability to capture the complex interactions among spatial layout and visual effects in real-world scenes. In particular, traditional 2D datasets do not provide the necessary geometric cues for accurately embedding text into diverse backgrounds. To address this limitation, we propose a novel standard for constructing synthetic datasets that incorporates surface normals to enrich three-dimensional scene characteristic. By adding surface normals to conventional 2D data, our approach aims to enhance the representation of spatial relationships and provide a more robust foundation for future scene text rendering methods. Extensive experiments demonstrate that datasets built under this new standard offer improved geometric context, facilitating further advancements in text rendering under complex 3D-spatial conditions.

==> sec/Figure_result_font.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{picture/F_compare3.png}
    \caption{Font Characteristic Preservation Comparison Between 2D and 3D Models}
    \label{fig:R_f}
\end{figure}

==> sec/Table_ppt.tex <==
\begin{table*}
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l cc cc cc}
      \toprule
      \multirow{2}{*}{Models}
        & \multicolumn{2}{c}{Total-Text}
        & \multicolumn{2}{c}{SVT}
        & \multicolumn{2}{c}{Syn3DTxt} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
      & $\mathrm{ACC}\!\uparrow$ & $\mathrm{ACC(80\%)}\!\uparrow$
      & $\mathrm{ACC}\!\uparrow$ & $\mathrm{ACC(80\%)}\!\uparrow$
      & $\mathrm{ACC}\!\uparrow$ & $\mathrm{ACC(80\%)}\!\uparrow$ \\
      \midrule
      InternVL3
        & {30.33} & {43.67}
        & {66.76} & {70.32}
        & {31.35} & {33.71} \\
      RolmOCR
        & \textbf{40.63} & \textbf{61.53}
        & \textbf{81.38} & \textbf{82.52}
        & \textbf{47.08} & \textbf{50.42} \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Quantitative results on Syn3DTxt-eval-2k, Syn3DTxt-wrap and Syn3DTxt-eval-advanced (only PSNR and SSIM shown). † indicates reproduced methods. Best two in each column are in \textbf{bold}.}
  \label{tab:comparison_table}
\end{table*}

